Benchmarking of Deep Learning Irradiance Forecasting Models from Sky Images -- an in-depth Analysis

A number of industrial applications, such as smart grids, power plant operation, hybrid system management or energy trading, could benefit from improved short-term solar forecasting, addressing the intermittent energy production from solar panels. However, current approaches to modelling the cloud cover dynamics from sky images still lack precision regarding the spatial configuration of clouds, their temporal dynamics and physical interactions with solar radiation. Benefiting from a growing number of large datasets, data driven methods are being developed to address these limitations with promising results. In this study, we compare four commonly used Deep Learning architectures trained to forecast solar irradiance from sequences of hemispherical sky images and exogenous variables. To assess the relative performance of each model, we used the Forecast Skill metric based on the smart persistence model, as well as ramp and time distortion metrics. The results show that encoding spatiotemporal aspects of the sequence of sky images greatly improved the predictions with 10 min ahead Forecast Skill reaching 20.4% on the test year. However, based on the experimental data, we conclude that, with a common setup, Deep Learning models tend to behave just as a 'very smart persistence model', temporally aligned with the persistence model while mitigating its most penalising errors. Thus, despite being captured by the sky cameras, models often miss fundamental events causing large irradiance changes such as clouds obscuring the sun. We hope that our work will contribute to a shift of this approach to irradiance forecasting, from reactive to anticipatory.

==> extra_references.tex <==
%author = {Modica, George D. and d'Entremont, R. and Mlawer, E. and Gustafson, G.},

@article{sirta,
  author = {Haeffelin, M.},
  title = {{Site instrumental de recherche par télédétection atmosphérique (Sirta)}},
  journal = {International Energy Agency (IEA)},
  year =         {2005}
}

@article{fchollet,
  author = {François Chollet},
  title = {{Deep Learning model with Python}},
  journal =    {Manning},
  year =         {2018}
}


@inproceedings{529922ff91eb49418849007453ba7edf,
title = "Constrained neural network for unconstrained handwritten digit recognition",
author = "Yann LeCun and B. Boser and Denker, {J. S.} and D. Henderson and Howard, {R. E.} and W. Hubbard and L.D. Jackel and Baird, {H. S.}",
year = "1990",
language = "English (US)",
editor = "C. Suen",
booktitle = "Frontiers in Handwriting Recognition, Montreal, 1990",
publisher = "CENPARMI, Concordia University",

}


@book{deep_learning,
  author =       {Ian Goodfellow, Yoshua Bengio, Aaron Courville},
  title =        {{Deep Learning model}},
  publisher =    {MIT press},
  year =         {2016}
}

@article{Resnet,
  author =       {Kaiming He, et al.},
  title =        {{Deep Residual Learning for Image Recognition}},
  publisher =    {Microsoft Research},
  year =         {2015},
  journal   =    {Arxiv}
}


@article{deep_conv,
  author =       {Szegedy, C. et al.},
  title =        {{Going deeper with convolutions}},
  journal =    {Conference on Computer Vision and Pattern Recognition (CVPR)},
  year =         {2015}
}

@article{very_dl,
  author =       {K.Simonyan and A. Zisserman},
  title =        {{Very deep convolutional networks for large-scale image recognition}},
  publisher =    {International Conference on Learning Representations (ICLR)},
  journal = {International Conference on Learning Representations (ICLR)},
  year =         {2015}
}


@article{dl_with_python,
  author =       {F. Chollet},
  title =        {{Deep Learning model with Python}},
  publisher =    {Manning},
  journal = {Manning},
  year =         {2018}
}

@article{Perez2013,
  author =       {R. Perez, T.E. Hoff},
  title =        {{Chapter 10 - SolarAnywhere Forecasting}},
  publisher =    {Academic Press, Boston},
  journal = {Solar Energy Forecasting and Resource Assessment},
  year =         {2013}
}


@MISC{Hinton2010,
    author = {Geoffrey E. Hinton},
    title = {Rectified Linear Units Improve Restricted Boltzmann Machines Vinod Nair},
    year = {2010}
}
